Faster Sampling without Isoperimetry via Diffusion-based Monte Carlo

To sample from a general target distribution $p_*\propto e^{-f_*}$ beyond the isoperimetric condition, Huang et al. (2023) proposed to perform sampling through reverse diffusion, giving rise to Diffusion-based Monte Carlo (DMC). Specifically, DMC follows the reverse SDE of a diffusion process that transforms the target distribution to the standard Gaussian, utilizing a non-parametric score estimation. However, the original DMC algorithm encountered high gradient complexity, resulting in an exponential dependency on the error tolerance $\epsilon$ of the obtained samples. In this paper, we demonstrate that the high complexity of DMC originates from its redundant design of score estimation, and proposed a more efficient algorithm, called RS-DMC, based on a novel recursive score estimation method. In particular, we first divide the entire diffusion process into multiple segments and then formulate the score estimation step (at any time step) as a series of interconnected mean estimation and sampling subproblems accordingly, which are correlated in a recursive manner. Importantly, we show that with a proper design of the segment decomposition, all sampling subproblems will only need to tackle a strongly log-concave distribution, which can be very efficient to solve using the Langevin-based samplers with a provably rapid convergence rate. As a result, we prove that the gradient complexity of RS-DMC only has a quasi-polynomial dependency on $\epsilon$, which significantly improves exponential gradient complexity in Huang et al. (2023). Furthermore, under commonly used dissipative conditions, our algorithm is provably much faster than the popular Langevin-based algorithms. Our algorithm design and theoretical framework illuminate a novel direction for addressing sampling problems, which could be of broader applicability in the community.

==> 0_config/init_load_colt_ver.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}         % Can be removed after putting your text content
\usepackage{graphicx}
\usepackage{natbib}
\usepackage{doi}
\usepackage{amssymb}
\usepackage{xcolor}         % colors
\usepackage{algorithm}
\usepackage{graphicx}
\usepackage{mathrsfs}
\usepackage{mathtools}% superior to amsmath
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{framed}
\usepackage{xspace}
\usepackage{enumitem}

\usepackage{algorithm2e}



% For paper revision:

\newcommand{\xh}[1]{\textcolor[HTML]{66CCFF}{#1}}
\def \dz {\textcolor{red}}

==> 0_config/math_commands_colt_ver.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newcommand{\hanze}[1]{{\textcolor{orange}{#1} }}

\newcommand{\issue}[1]{{\textcolor{purple}{#1} }}
% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rvzeta{{\mathbf{\zeta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\cR{{\mathcal{R}}}
\def\EE{{\mathbb{E}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vrho{{\bm{\rho}}}
\def\vzeta{{\bm{\zeta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

%

\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {\tiny{#1}};}}
% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}[2]{\mathrm{KL}\left(#1 \| #2\right)}
\newcommand{\FI}[2]{\mathrm{FI}\left(#1 \| #2\right)}
\newcommand{\TVD}{D_{\mathrm{TV}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


\newcommand{\der}{\mathrm{d}}
\newcommand{\fder}{\mathrm{D}}
\newcommand{\rgrad}{\mathrm{grad}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% Table settings

\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother

\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{3\arrayrulewidth}

\newcommand{\tabitem}{~~\llap{\textbullet}~~}


%Specific Notations for Sampling along the Reverse Process with Recursive Score Estimation

\newcommand{\rbkwx}{\rvx^{\gets}}
\newcommand{\bkwx}{\vx^{\gets}}
\newcommand{\rbkwv}{\rvv^{\gets}}
\newcommand{\bkwp}{p^{\gets}}
\newcommand{\ourmethod}{\text{RS-DMC}}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}
\newcommand{\lIfElse}[3]{\lIf{#1}{#2 \textbf{else}~#3}}

==> 0_contents/010introduction_backup.tex <==
\section{Introduction}

The recent success of diffusion models (DMs) has shown great potential for generating samples from complex distributions, both in practical applications~\cite{ho2020denoising, rombach2021highresolution} and in theoretical research~\cite{chen2022sampling, chen2023improved}.
Given a series of well-trained time-dependent score estimations, the inference process of DMs can be viewed as gradient-based MCMC sampling methods that discretize a reverse Ornstein-Uhlenbeck (OU) process starting from the data distribution.
However, it is unclear whether the inference process can be extended to the Monte Carlo sampling (MCS) problem and what improvements can be achieved.


One challenge is that MCS and DMs have opposite known conditions.
Specifically, DMs require drawing samples from an unknown distribution, given several samples that follow this distribution.
In contrast, MCS requires drawing samples from the target distribution $p_*\propto \exp(-f_*)$ with an analytic form, without any given samples.
To sample along the reverse OU process in the inference process, DMs parameterize the score of the target density with neural networks and train the model with additional samples (training set) whose underlying distribution is $p_*$.
If some non-parametric methods can replace this score estimation process when the unnormalized target density is given, then the feasibility of extending DMs to MCS can be addressed.
Considering the ability of DMs to handle complex target distributions, we expect that their extension to MCS will converge in more general targets compared with existing gradient-based Markov chain Monte Carlo (MCMC) methods, e.g., Unadjusted Langevin Algorithm (ULA)~\cite{vempala2019rapid}, Underdamped Langevin Dynamics (ULD)~\cite{cheng2018convergence} and Metropolis-Adjusted Langevin Algorithm (MALA)~\cite{dwivedi2018log}.



Several recent studies, including~\cite{montanari2023sampling, huang2023monte}, have attempted to estimate the score and simulate the inference process in DMs to address MCS tasks.
Specifically,~\cite{huang2023monte} proposed a non-parametric score estimation method called RDS, which is based on an inner-loop ULA.
They proved that the total variation distance to the target distribution converges beyond the Poincar\'e inequality requirement of the target.
However, their assumptions are covered by weak Poincar\'e inequality that guarantees ULA convergence, as shown in~\cite{mousavi2023towards}.
Although RDS overcomes the exponential dimensionality dependency that ULA suffers from in general heavy-tail cases, it still has an exponential approximate error dependency. 
In other words, RDS is better suited for high-dimensional MCS tasks that require a moderate total variation distance to the target distribution.
These results motivate us to ask
\begin{framed}
    \centering
    \it Can an exponential dependence-free convergence be achieved beyond isoperimetry by a reverse OU process? 
\end{framed}

To address the problem mentioned above, we propose a novel non-parametric method for score estimation. 
We divide the entire forward process into several segments and estimate the score at time $t$ using Tweedie’s formula.
In the formula, the conditional probability is the transition kernel of the forward process (i.e., OU process) from the starting point of the segment $t$ located at time $t^\prime$ to $t$, rather than starting from the beginning of the entire process (at time $0$) to $t$, as done in~\cite{huang2023monte}.
Compared with the time $0$, time $t^\prime$ will be much closer to $t$, making the estimation much easier.
For exchange, to use Tweedie's formula, we need to estimate the score at time $t^\prime$ because it does not have an analytical form like the score at time $0$, which is given by the target distribution as $\grad\ln p_*$.
This leads us to introduce a recursive method to estimate the score at time $t$, $t^\prime$, etc.
However, by choosing the segment length appropriately, we can trade off the complexity of the score estimation at time $t$ and its corresponding recursive calls and finally obtain a better gradient complexity.
Surprisingly, when the segment length is some constant, our estimation will lead to a Kullback–Leibler (KL) convergence that only requires the second moment bound and log density smoothness rather than any isoperimetry of the target distribution $p_*$, including weak Poincar\'e inequality.
Furthermore, we prove that the gradient complexity required to achieve the KL convergence does not have exponential dependency for both the dimensionality and approximate error.
Some additional works share the same assumption with ours, e.g.,~\cite{balasubramanian2022towards}, while they can only provide the Fisher information convergence. 
To the best of our knowledge, this is the first work for gradient-based MCMC algorithms to KL converge beyond isoperimetry and even with a better dimensional dependence in gradient complexity compared with ULA in weak Poincar\'e inequality~\cite{mousavi2023towards}.

The main contributions of this paper can be summarized in the following three perspectives:
\begin{itemize}
    \item We propose a novel non-parametric method for the score estimation and combine it with the reverse diffusion process to create an efficient gradient-based MCMC method.
    To simplify the difficulty of the sampling subproblem for score estimation, we introduce a recursive process conducted on the segmented forward process.
    By tuning the length of segments, we balance the difficulty of subproblems and the number of recursive calls.
    \item From a theoretical perspective, we prove that our method achieves KL convergence even when the target distribution only satisfies the second moment bound and log density smoothness rather than any isoperimetry. 
    Furthermore, we show the gradient complexity required to achieve such convergence is $(d/\epsilon)^{\mathcal{O}(\ln (1/\epsilon))}$, without any exponential dependency on the dimensionality and approximate error.
    Traditional gradient-based MCMC methods can only achieve Fisher information convergence under the same assumptions.
    Even in general weak Poincar\'e inequality settings, our proposed method achieves a better dimensional dependency in gradient complexity compared with ULA~\cite{mousavi2023towards}.
    \item \textcolor{blue}{Maybe we can show some empirical results to make our work more solid.}
\end{itemize}


==> 0_contents/030method_colt.tex <==
\section{Proposed Methods}
\label{sec:method}

In this section, we introduce a new approach called Recursive Score Estimation (RSE) and describe the proposed Recursive Score Diffusion-based Monte Carlo (RS-DMC) method.
We start by discussing the motivations and intuitions behind the use of recursion.
Next, we provide implementation details for the RSE process and emphasize the importance of selecting an appropriate segment length.
Finally, we present the RS-DMC method based on the RSE approach.

\subsection{Difficulties of the vanilla DMC}
% \textcolor{red}{Add a section about the difficulty of the vanilla reverse diffusion Monte Carlo. Stress the problem with score estimation away from $p_{0,0}$. Then connect to the intuition of why recursion would help.}

We consider the reverse segmented OU process, i.e., SDE~\ref{con_eq:rrds_actual_backward} and begin with the original version of DMC in \citet{huang2023monte}, which can be seen as a special case of the reverse segmented OU process with a large segment length $S=T$ and a small number of segments $K=1$.
According to the reverse SDE~\ref{con_eq:rrds_actual_backward}, for the $r$-th iteration within one single segment, we need to estimate $\grad\log p_{0,S-r\eta}$ to update the particles.
Specifically, by Lemma~\ref{con_lem:score_reformul}, we have
\begin{equation*}
    \grad \log p_{0,S-r\eta}(\vx) = \mathbb{E}_{\rvx_0 \sim q_{0, S-r\eta}(\cdot|\vx)}\left[-\frac{\vx - e^{-(S-r\eta)}\vx_0}{\left(1-e^{-2(S-r\eta)}\right)}\right]
\end{equation*}
for any $\vx\in\R^d$, where the conditional distribution $q_{0, S-r\eta}(\cdot |\vx)$ is
\begin{equation}
    \label{eq:tar_axu_dis}
    \small
    q_{0,S-r\eta}(\vx_0|\vx) \propto \exp\bigg( \log p_{0,0}(\vx_0)-\frac{\left\|\vx - e^{-(S-r\eta)}\vx_0\right\|^2}{2\left(1-e^{-2(S-r\eta)}\right)}\bigg).
\end{equation}
Since the analytic form $\grad\log p_{0, 0}=-f_*$ exists, we can use the ULA to draw samples from $q_{0, S-r\eta}(\cdot|\vx)$ and calculate the empirical mean to estimate $\grad\log p_{0,S-r\eta}(\vx)$.

However, sampling from $q_{0, S-r\eta}(\cdot|\vx)$ is not an easy task. When $r$ is very small, sampling $q_{0,S-r\eta}(\cdot|\vx)$ via ULA is almost as difficult as sampling $p_{0,0}(\vx_0)$ via ULA (see \eqref{eq:tar_axu_dis}), since the additive quadratic term, whose coefficient is $e^{-2(S-r\eta)}/2(1-e^{-2(S-r\eta)})$, will be nearly negligible in this case. This is because that $S=T$ is large and then $e^{-2(S-r\eta)}/2(1-e^{-2(S-r\eta)})\sim \exp(-2T)$ becomes extremely small when $r\eta=O(T)$.
More specifically, as shown in \citet{huang2023monte}, when $e^{-2(S-r\eta)}\le 2L/(1+2L)$, the LSI parameter of $q_{0,S-r\eta}(\cdot|\vx)$ can be as worse as $\exp\big(-\mathcal O(1/\epsilon)\big)$. Then applying ULA for sampling this distribution needs a dramatically high gradient complexity that is exponential in $1/\epsilon$.




% Compared to sampling directly from the target density $p_* = p_{0,0} \propto \exp(-f_*)$, the log density of $q_{0,S-r\eta}(\cdot|\vx)$ only adds an additional quadratic regularizer, whose coefficient is small when $r$ is close to $0$.
% Although such a quadratic term helps provide the LSI property for $q_{0, S-t}(\cdot|\vx)$ when $p_*$ is heavy-tailed in some cases, the LSI constant will be highly affected by the quadratic coefficient or the choice of $S$.
% In general, $T=S$ is at the $\log(1/\epsilon)$ level. 
% It will cause the LSI constant to be extremely small and at the $\mathcal{O}\big(\frac{1}{\exp(1/\epsilon)}\big)$ level as shown in~\cite{huang2023monte}, 

\subsection{Intuition of the recursion}

Therefore, the key to avoiding sampling such a hard distribution is to restrict the segment length. By Lemma \ref{con_lem:score_reformul}, it can be straightforwardly verified that if the segment length satisfies $S\le \frac{1}{2}\log\left(\frac{2L+1}{2L}\right)$, 
% To alleviate the difficulty of the sampling subproblem to estimate the score,  we choose a small segment length when approximating $\grad\log p_{k,S-r\eta}(\vx)$, which makes $q_{k, S-r\eta}(\cdot|\vx)$ strongly log-concave.
% Specifically, by choosing , 
% we have
\begin{equation}
    \label{con_ineq:cho_s_small}
    -\grad_{\vx_0}^2\log q_{k,S-r\eta}(\vx_0|\vx) \succeq -\grad^2_{\vx_0} \log p_{k,0}(\vx_0)+ \frac{e^{-2S}}{1-e^{-2S}}\cdot \mI \succeq \frac{e^{-2S}}{2(1-e^{-2S})}
\end{equation}
where the last inequality follows from Assumption~\ref{con_ass:lips_score}.
This implies that $q_{k,S-r\eta}(\vx_0|\vx)$ is strongly log-concave for all $r\le \lfloor S/\eta\rfloor$, which can be efficiently sampled via the standard ULA. However, ULA requires to calculate the score function  $\nabla_{\vx_0} \log q_{k,S-r\eta}(\vx_0|\vx)$, which further needs to calculate $\nabla\log p_{k,0}(\vx)$ according to Lemma \ref{con_lem:score_reformul}. Different from the vanilla DMC where the formula of $\nabla \log p_{0,0}(\vx)$ is known, the score $\nabla\log p_{k,0}(\vx)$ in \eqref{con_ineq:cho_s_small} is an unknown quantity, which also requires to be estimated. In fact, based on our definition, we can rewrite $p_{k,0}(\vx)$ as $p_{k-1,S}(\vx)$ (see Figure \ref{con_fig:rrds_forward}), then applying Lemma \ref{con_lem:score_reformul}, we can again decompose the problem of estimating $\nabla \log p_{k-1,S}(\vx)$ into the subproblems of sampling $q_{k-1, S}(\cdot|\vx)$ and the estimation of $\nabla \log p_{k-1,0}(\vx)$, which is naturally organized in a recursive manner. Therefore, by recursively adopting this subproblem decomposition, we summarize the recursive process for approximating $\grad\log p_{k,S-r\eta}(\vx)$ as follows and illustrate the diagram in Figure \ref{con_fig:rse}: 
% While as a price of sampling from a strongly log-concave $q_{k,S-r\eta}(\cdot|\vx)$, we cannot use ULA directly because an unknown term, i.e., $\grad\log p_{k,0}$ is included in $\grad\log q_{k,S-t}(\cdot|\vx)$ which dominates the velocity in particles' updating.
% However, due to SDE~\ref{con_eq:rrds_forward}, we can approximate the score $\grad\log p_{k,0}=\grad\log p_{k-1,S}$ using Lemma~\ref{con_lem:score_reformul} with the previous segment, i.e., the $(k-1)$-th segment, until $k=0$.

%\textcolor{red}{Rewrite the paragraph above (see whether GPT4 can generate a reasonable paragraph).}
%\textcolor{red}{Also we are actually sampling $q_{k, S-t}(\cdot|\vx)$ via the forward SDE~\ref{con_eq:rrds_forward}, instead of ULA?}
\begin{itemize}[leftmargin=*,nosep]
    \item \textbf{Step 1:} We approximate the score $\grad\log p_{k,S-r\eta}(\vx)$ by a mean estimation with samples generated by running ULA over the intermediate target distribution $q_{k, S-r\eta}(\cdot|\vx)$.
    \item \textbf{Step 2:} When running ULA for $q_{k, S-t}(\cdot|\vx)$, we estimate the score $\grad\log p_{k,0} = \grad\log p_{k-1,S}$.
    \item \textbf{Step 3:} We jump to Step~1 to approximate the score $\grad\log p_{k-1,S}(\vx)$ via drawing samples from $q_{k-1, S}(\cdot|\vx)$, and continue the recursion.
\end{itemize}
% This recursive process is illustrated in Fig~\ref{con_fig:rse}.
\begin{figure}
    \centering
    \input{0_figs/recursion_explain}
    \vspace{-.1in}
    \caption{\small The illustration of recursive score estimation (RSE).
    The upper half presents RSE from a local view, which shows how to utilize the former score, e.g., $\grad\log p_{k,0}(\vx^\prime)$ to update particles by ULA in the sampling subproblem formulated by the latter score, e.g., $\grad\log p_{k,S-t}(\vx)$. The lower half presents RSE from a global view, which is a series of interconnected mean estimation and sampling subproblems accordingly.}
    \label{con_fig:rse}
    \vspace{-.1in}
\end{figure}

\subsection{Recursive Score Estimation and Reverse Diffusion Sampling}

\noindent\textbf{Recursive Score Estimation.}
In the previous section, we explained the rough intuition behind introducing recursion. By conducting the recursion, we need to solve a series of sampling and mean estimation subproblems. Then, it is demanding to control the error propagation between these subproblems in order to finally ensure small sampling errors. In particular, this amounts to the adaptive adjustment of the sample numbers for mean estimation and iteration numbers for ULA in solving sampling subproblems.
% Before formally stating the recursive score estimation (RSE) algorithm, we need to adaptively adjust the sample number for mean estimation and the iteration number for the sampling subproblems (i.e., ULA), in order to control the error propagation in the recursion. 
%\textcolor{red}{(In the above sentence, just say that we specify the requirements of the number of samples/gradient queries. Don't start the sentence with "however".)}
Specifically, if we require score estimation $\rbkwv_{k,r\eta}\colon \R^d\rightarrow \R^d$ to satisfy
\begin{equation}
    \label{ineq:score_req}
    \left\|\grad\log p_{k,S-r\eta}(\vx) - \rbkwv_{k,r\eta}(\vx)\right\|^2\le \epsilon,\ \forall \vx\in\R^d
\end{equation}
with a high probability, then the sample number in Step 1 and the number of calls of Step 2 (the iteration number of ULA) in Fig~\ref{con_fig:rse} will be 
two functions with respected to the target error $\epsilon$, denoted as $n_{k,r}(\epsilon)$ and $m_{k,r}(\epsilon)$ respectively.
Furthermore, when Step 2 is introduced to update ULA, we rely on an approximation of $\grad\log p_{k,0}$ instead of the exact score. 
To ensure \eqref{ineq:score_req} is met, the error resulting from estimating $\grad\log p_{k,0}$ should be typically smaller than $\epsilon$. We express this requirement as:
\begin{equation*}
    \left\|\grad\log p_{k,0}(\vx) - \rbkwv_{k,0}(\vx)\right\|^2\le l_{k,r}(\epsilon),\ \forall \vx\in\R^d.
\end{equation*}
where $l_{k,r}(\epsilon)$ is a function of $\epsilon$ that satisfies $l_{k,r}(\epsilon)\le \epsilon$.
Under this condition, we provide Alg~\ref{con_alg:rse}, i.e., RSE, to calculate the score function for the $r$-th iteration at the $k$-th segment, i.e., $\grad\log p_{k,S-r\eta}(\vx)$.

\begin{algorithm}[t]
    \SetAlgoLined
    \SetNoFillComment
    \LinesNumbered 
    \KwData{The segment number $k\in \mathbb{N}_{0, K-1}$, the iteration number $r\in\mathbb{N}_{0,R-1}$, variable $\vx$ requiring the score function, error tolerance $\epsilon$.} 
    \uIf{$k\equiv -1$}{
        \Return $-\grad f_*(\vx)$\; \label{con_alg:rse_score_ret_condi}
    } 
    Initial the returned vector $\vv^\prime \gets \vzero$\;
    
    \For{$i=1$ to $n_{k,r}(\epsilon)$}{
        Draw $\vx^\prime_0$ from an initial distribution $q^\prime_0$\;
        
        \For{$j=0$ to $m_{k,r}(\epsilon,\vx)-1$}{
            $\vv^\prime_j \gets \mathsf{RSE}\left(k-1, 0, \vx^\prime_{j}, l_{k,r}(\epsilon)\right)$\;
            \tcc{Recursive score estimation $\grad\log p_{k-1,S}(\vx^\prime_{j})$}

            \lIfElse{$r\not\equiv 0$}
            {
                $t^\prime \gets S-r\eta$\;
            }
            {
                $t^\prime \gets S$\;
            } 
            \tcc{The gap of time since the last call}
            Update the particle 
            \begin{equation*}
                \vx^\prime_{j+1}\coloneqq \vx^\prime_{j}+\tau_r\cdot \underbrace{\bigg(\vv^\prime_j + \frac{e^{-t^\prime}\vx - e^{-2t^\prime}\vx^\prime_{j}}{1-e^{-2t^\prime}} \bigg)}_{\approx \grad\log q_{k,S-r\eta}(\vx^\prime_{j}|\vx)} +\sqrt{2\tau_r}\cdot \xi
            \end{equation*}\;
        }
        Update the score estimation of $\vv^\prime\approx \grad\log p_{k,S-r\eta}(\vx)$ with empirical mean as $$\vv^\prime \coloneqq \vv^\prime + \frac{1}{n_{k,r}(\epsilon)}\bigg(-\frac{\vx - e^{-t^\prime}\vx_{m_{k,r}(\epsilon)}^\prime}{1-e^{-2t^\prime}}\bigg)$$\;   
    }
    \Return $\vv^\prime$\; \tcc{As the approximation of $\grad\log p_{k,S-r\eta}(\vx)$}                
    \caption{Recursive Score Estimation (approximate $\grad\log p_{k,S-r\eta}(\vx)$): $\mathsf{RSE}(k,r,\vx,\epsilon)$}
    \label{con_alg:rse}
\end{algorithm}

\noindent\textbf{Quasi-polynomial Complexity.} We consider the ideal case for interpreting the complexity of our score estimation method. In particular, since the benign error propagation, i.e., $l_{k,r}(\epsilon)=\epsilon$, is almost proven in Lemma~\ref{lem:recursive_core_lem}, we suppose the number of calls to the recursive function, $\mathsf{RSE}(k-1,0,\vx^\prime,l_{k,r}(\epsilon))$, is uniformly bounded by $m_{k,r}(\epsilon)\cdot n_{k,r}(\epsilon)$ for all feasible $(k,r)$ pairs when the RSE algorithm is executed with input $(k,r,\vx,\epsilon)$.
Then, recall that we will conduct the recursion in at most $K$ rounds, the total gradient complexity for estimating one score will be 
\begin{equation*}
    \left[m_{k,r}(\epsilon)\cdot n_{k,r}(\epsilon)\right]^{\mathcal{O}(K)} = \left[m_{k,r}(\epsilon)\cdot n_{k,r}(\epsilon)\right]^{\mathcal{O}(T/S)}. 
\end{equation*}
This formula highlights the importance of selecting a sufficiently large segment with length $S$ to reduce the number of recursive function calls and improve gradient complexity.
% While a large $S$ leads to the failure of strong convexity for the auxiliary\xunp{should be removed} distribution $q_{k,S-r\eta}$ demonstrated in \eqref{con_ineq:cho_s_small}.
% Therefore, the segment length $S$ can be regarded as a hyper-parameter that balances the challenges of score estimation and recursive calls.
In our analysis, we set $S=\frac{1}{2}\log\left(\frac{2L+1}{2L}\right)$, which is ``just'' small enough to ensure that all intermediate target distributions in the sampling subproblems are strongly log-concave.
In this condition, due to the choice of $T$ is $\mathcal{O}(\log (d/\epsilon))$ in general cases and $m_{k,r}(\cdot)$ and $n_{k,r}(\cdot)$ are typically polynomial w.r.t. the target sampling error $\epsilon$ and dimension $d$ (see Theorem~\ref{thm:main_rrds_formal} in Appendix~\ref{app_sec:main_proof}), we would expect a quasi-polynomial gradient complexity. 

\noindent\textbf{Diffusion-based Monte Carlo with Recursive Score Estimation.}
Then based on the RSE algorithm in Alg \ref{con_alg:rse}, we can directly apply the DDPM \citep{ho2020denoising} based method to perform the sampling, giving rise to the Recursive Score Diffusion-based Monte Carlo (RS-DMC) method. We summarize the proposed RS-DMC algorithm in Alg~\ref{alg:rrds} (the detailed setup of $m_{k,r}(\cdot)$, $n_{k,r}(\cdot)$, $l_{k,r}(\cdot)$ are provided in Theorem~\ref{thm:main_rrds_formal} in Appendix~\ref{app_sec:main_proof}).

% \noindent\textbf{Discussion on the Complexity Improvements.} \textcolor{blue}{
% The Bayesian inference problem can oftentimes be cast as the problem of estimating the posterior mean of certain function (e.g., prediction output, its higher moments, or quantile functions). 
% The question factorizes into two parts: a posterior sampling problem, and a mean estimation problem.
% The mean estimation problem is relatively well understood, given some mild assumptions on the tail of the posterior distribution (e.g., sub-Gaussianity or moment bounds).
% The posterior sampling problem without the isoperimetric assumptions has eluded conclusive results, despite century-long endeavors.
% The existing convergence upper bounds of the MCMC algorithms are exponential in the dimension of the problems.
% This poses an exponential gap between the posterior sampling problem and the mean estimation problem.}

% \textcolor{blue}{
% In this work, we propose that one can translate the posterior sampling problem into a mean estimation problem plus a log-concave sampling problem, which enjoys polynomial convergence rates.
% We thereby obtain a convergence rate that has sub-exponential dependence on the dimension of the problem.
% This provides an exponential improvement over the existing results in the posterior sampling literature.
% }


\begin{algorithm}
    \caption{Recursive Score Diffusion-based Monte Carlo (RS-DMC)}
    \label{alg:rrds}
    \begin{algorithmic}[1]
            \State {\bfseries Input:} Initial particle $\rbkwx_{K,S}$ sampled from $p_\infty$, Terminal time $T$, Step size $\eta$, required convergence accuracy $\epsilon$;
            \For{$k=K-1$ down to $0$}
                \State Initialize the particle as $\bkwx_{k,0} \gets  \bkwx_{k+1, S}$
                \For{$r=0$ to $R-1$}
                    \State Approximate the score, i.e., $\grad\log p_{k,S-r\eta}(\bkwx_{k,r\eta})$ by $\vv^\prime \gets \mathsf{RSE}(k,r,\bkwx_{k,r\eta},l(\epsilon))$
                    \State $\bkwx_{k, (r+1)\eta} \gets e^\eta\bkwx_{k,r\eta}+\left(e^\eta - 1\right)\vv^\prime +\xi$ where $\xi$  is sampled from  $\mathcal{N}\left(0,  \left(e^{2\eta}-1\right)\mI_d\right)$
                \EndFor
            \EndFor
            \State {\bfseries Return:} $\bkwx_{0,S}$.
    \end{algorithmic}
\end{algorithm}
    


==> 0_contents/050relatedwork.tex <==
\section{Related Work}

==> 0_contents/backup.tex <==
\begin{algorithm}
    \caption{Coarse-grained Recursive Score Estimation (approximate $\grad\ln p_{k,0}(\vx)$)}
    \label{con_alg:c_rse}
    \begin{algorithmic}[1]
            \STATE {\bfseries Input:} The segment number $k$, variable $\vx$ requiring the score function, error tolerance $\epsilon$;
            \IF{$k\equiv 0$ }
                \STATE {\bfseries Return:} $-\grad f_*(\vx)$. 
            \ENDIF
            \STATE Initial the returned vector $\vv^\prime = \vzero$;
            \FOR{$i = 1$ to $n_{k,0}(\epsilon)$}
                \STATE Draw a particle $\vx_0^\prime$ from initial distribution $q^\prime_{0}$;
                \FOR{$j = 0$ to $m_{k,0}(\epsilon)-1$}
                    \STATE Approximate $\grad\ln p_{k-1,0}(\vx^\prime_{j})$ with $\vv^\prime_j \coloneqq \mathrm{Alg~\ref{con_alg:c_rse}}(k-1,\vx^\prime_{j}, l_{k,0}(\epsilon))$;
                    \STATE Update the particle
                    \begin{equation*}
                        \small
                        \vx_{j+1}^\prime \coloneqq \vx_{j}^\prime + \tau\cdot \underbrace{\left(\vv_j^\prime + \frac{e^{-S}\vx - e^{-2S}\vx^\prime_j}{1-e^{-2S}}\right)}_{\approx \grad\ln q_{k,0}(\vx_j^\prime|\vx)} + \sqrt{2\tau}\cdot \xi
                    \end{equation*}
                \ENDFOR
                \STATE Update the score estimation of $\vv^\prime\approx \grad\ln p_{k,0}(\vx)$ with empirical mean as $$\vv^\prime \coloneqq \vv^\prime + \frac{1}{n_{k,0}(\epsilon)}\left(-\frac{\vx - e^{-S}\vx_{m_{k,0}(\epsilon)}^\prime}{1-e^{-2S}}\right)$$
            \ENDFOR
            \STATE {\bfseries Return:} $\vv^\prime$.
    \end{algorithmic}
\end{algorithm}



\subsection{Recursively Reverse Diffusion Sampling}
By implementing the RSE technique in the reverse sampling framework introduced in~\cite{huang2023monte}, we have developed a new sampling algorithm called Recursively Reverse Diffusion Sampling (RRDS), which updates particles along the reverse OU process in Alg~\ref{alg:rrds} where $l(\epsilon)$ denotes the error tolerance of score estimations when the required convergence accuracy is $\epsilon$.

\begin{theorem}
    \label{thm:main_rrds}
    Assume the target distribution $p_*$ satisfies Assumption~\ref{con_ass:lips_score}-\ref{con_ass:second_moment}, and $L\ge 1$ without loss of generality, we suppose 
    \begin{equation*}
        \begin{aligned}
            &S=\frac{1}{2}\ln\left(\frac{2L+1}{2L}\right),\quad  \eta=C_{\eta}\cdot (d+m_2^2)^{-1}\epsilon,\quad \tau_r = C_\tau\cdot (1-e^{-2(S-r\eta)})^2e^{2(S-r\eta)}d^{-1}\epsilon\\
            & l_{k,r}(\epsilon)=C_l\cdot \epsilon,\quad \quad m_{k,r}(\epsilon)=C_m\cdot (d+m_2^2)^{3}\epsilon^{-3}\max\{\ln Z^2,1\},\\
            &\mathrm{and}\ n_{k,r}(\epsilon)=C_n\cdot (d+m_2^2)\epsilon^{-2}\cdot\max\left\{d, \left(\ln \left((d+m_2^2)/\epsilon\right)\right)^3\right\}
        \end{aligned}
    \end{equation*}
    where the constants, i.e., $C_\eta, C_\tau, C_l, C_m, C_n$, are independent with $d$, $m_2$ and $\epsilon$.
    To simplify the notation, $Z$ denotes the maximum norm of particles which appears in Alg~\ref{alg:rrds}.
    Then, we have 
    \begin{equation*}
        \KL{p_*}{\bkwp_{0,S}} =\tilde{\mathcal{O}}(\epsilon)
    \end{equation*}
    with a probability at least $1-\epsilon$.
    In this condition, the gradient complexity will be 
    \begin{equation}
        \label{eq:converge_rrds_sm}
        \begin{aligned}
            &\mathrm{poly}\left(\frac{Ld+m_2^2}{\epsilon^2}, \ln\frac{Ld+m_2^2}{\epsilon}\cdot \max\left\{\ln\ln Z^2,1\right\}\right)\\
            & \exp\left(\mathcal{O}\left(\ln \frac{Ld+m_2^2}{\epsilon}\right)\right)
        \end{aligned}
    \end{equation}
\end{theorem}




%--------------- section 4 revision

when the target distribution $p_*\propto \exp(-f_*)$ satisfies the following assumptions:
\begin{itemize}
    \item The function $f_*$ takes nonnegative real values, and there exist constants $A,B\ge 0$, such that $|f_*(\vzero)|\le A$ and $\|\grad f_*(\vzero)\|\le B$.
    \item The function $f_*$ is $L$-smooth: for some $L>0$, $\|\grad f_*(\vx)-\grad f_*(\vx^\prime)\|\le L\|\vx-\vx^\prime\|$.
    \item The function $f_*$ is $(m,b)$-dissipative~\cite{hale2010asymptotic}: for some $m>0$ and $b\ge 0$, $\left<\vx, \grad f_*(\vx)\right>\ge m\left\|\vx\right\|^2-b,\forall \vx\in\R^d$.
\end{itemize}
The LSI constant only has the following bound $\mu^{-1} = \exp(\tilde{\mathcal{O}}(d))$ as shown in~\cite{raginsky2017non}.
In this condition, Eq~\ref{eq:converge_ula_lsi} becomes $\mathcal{O}(L^2 \cdot d\epsilon^{-1})\cdot \exp(\tilde{O}(d))$ which is significantly worse than Eq~\ref{eq:converge_rrds_sm} for high-dimensional targets.

\cite{balasubramanian2022towards} considers the case when the negative log density, i.e., $f_*$ is possibly non-convex but $L$-smooth, they prove that a variant of ULA named averaged Langevin Monte Carlo outputs a sample with $\epsilon$-relative Fisher information, i.e., $\FI{p}{p_*}\coloneqq \E_{p}[\left\|\grad\ln (p/p_*)\right\|^2]$, with $\mathcal{O}(L^2d^2\epsilon^{-2})$ gradient complexity.
Compared with our result, they do not require the second moment bound, i.e.,~\ref{con_ass:second_moment}.
However, unlike the situation in non-convex optimization, in sampling, there are no "spurious stationary points": if $p$ and $p_*$ have positive and smooth densities and $\FI{p}{p_*}=0$, then $p=p_*$. 
However, for $\epsilon>0$ it may be unclear what the guarantee $\FI{p}{p_*}\le \epsilon$ entails.
They have proved that, in some cases, even if the Fisher information $\FI{p}{p_*}$ is very small, the total variation distance remains bounded away from zero.
In the Theorem~\ref{alg:rrds}, the criterion of \ourmethod can easily upper bound the TV between $p_*$ and the underlying distribution of output particles by Pinsker's inequality~\cite{csiszar2011information}.

\paragraph{Comparison with RDS.} Actually, \ourmethod shares the same continuous process with RDS proposed in~\cite{huang2023monte}.
However, we introduce RSE, i.e., Alg~\ref{con_alg:rse}, which estimates the score in a more clever way.
From the theoretical perspective, we have improved both in weakening assumptions and strengthening conclusions.
Besides the requirement of~\ref{con_ass:lips_score} and~\ref{con_ass:second_moment}, in~\cite{huang2023monte}, the target distribution additionally requires the polynomial growth assumption for the negative log density as follows:
\begin{itemize}
    \item For any $r>0$, we can find some $R(r)$ satisfying $f_*(\vx)+\delta\left\|\vx\right\|^2$ is convex for $\left\|\vx\right\|\ge R(r)$. Without loss of generality, we suppose $R(r) = c_R/r^n$ for some $n>0,c_R>0$.
\end{itemize}
This assumption guarantees the target distribution of the auxiliary subproblem, i.e., $q_{0,S-r\eta}(\cdot|\vx)$, in Eq~\ref{eq:tar_axu_dis}, to satisfy LSI. 
Although the LSI constant of $q_{0,S-r\eta}(\cdot|\vx)$ can get rid of the exponential dependence of $d$, for exchange, it will have additional factor of $\exp((1/\epsilon)^{\mathcal{O}(n)})$.
It causes the total gradient complexity for the KL convergence to be 
\begin{equation*}
    \mathrm{poly}(d)\cdot \mathrm{poly}(1/\epsilon)\cdot \exp\left(\mathcal{O}(1/\epsilon)\right).
\end{equation*}
By choosing the appropriate segment length $S$ and balancing the challenges of score estimation and recursive calls with RSE, \ourmethod not only naturally removes the tail-growth assumption but also improves the gradient complexity.


\subsection{Proof Sketch}

In this section, we aim to highlight the technical innovations by presenting the roadmap of our analysis. Due to space constraints, we have included the technical details in the Appendix.

Firstly, we can establish an upper bound on the KL divergence gap between the target distribution $p_*$ and the underlying distribution of output particles, i.e., $\bkwp_{0,S}$, as follows:
\begin{equation*}
    \KL{p_*}{\bkwp_{0,S}}\le \underbrace{\KL{p_{K-1,S}}{\bkwp_{K-1,0}}}_{\text{Term 1}}+\E_{\rvx\sim 0_{K-1,S}}\left[\KL{p_{(0,0)|(K-1,S)}(\cdot|\rvx)}{\bkwp_{(0,S)|(K-1,0)}(\cdot|\rvx) }\right].
\end{equation*}

\paragraph{Upper bound Term 1.}
The first term can be bounded using exponential mixing
of the forward (Ornstein-Uhlenbeck) process towards the
standard Gaussian in Lemma~\ref{lem:var_thm4_vempala2019rapid}, i.e., 
\begin{equation*}
    \KL{p_{K-1,S}}{\bkwp_{K-1,0}}\le \KL{p_*}{\bkwp_{K-1,0}}\exp(-KS) \le  (d+m_2^2)\exp(-KS),
\end{equation*}
where $\bkwp_{K-1,0}=\mathcal{N}(\vzero, \mI)$ as shown SDE~\ref{con_eq:rrds_actual_backward}.

For the remaining term, we compare the continuous process with the estimated, discrete process through a chain of intermediate processes.
By utilizing the chain rule for KL divergence, we can express this term as a sum.
We can interpolate the discrete processes to represent them as SDEs. If Novikov's conditions are satisfied, Girsanov's Theorem can be utilized to restrict the KL divergence in relation to the squared difference of the drift terms between the processes.
\begin{equation*}
    \begin{aligned}
        &\E_{\rvx\sim 0_{K-1,S}}\left[\KL{p_{(0,0)|(K-1,S)}(\cdot|\rvx)}{\bkwp_{(0,S)|(K-1,0)}(\cdot|\rvx) }\right]\\
        & \le \underbrace{2\sum_{k=0}^{K-1}\sum_{r=0}^{R-1} \int_{0}^\eta \E_{(\rbkwx_{k,t+r\eta}, \rbkwx_{k,r\eta})}  \left[\left\|\grad\ln p_{k, S-(t+r\eta)}(\rbkwx_{k,t+r\eta}) - \grad\ln p_{k,S-r\eta}(\rbkwx_{k,r\eta}) \right\|^2\right]\der t}_{\text{Term 2}}\\
        & \quad + \underbrace{2\sum_{k=0}^{K-1}\sum_{r=0}^{R-1} \int_{0}^\eta \E_{\rbkwx_{k,r\eta}}\left[\left\|\grad\ln p_{k,S-r\eta}(\rbkwx_{k,r\eta})- \rbkwv_{k,r\eta}(\rbkwx_{k,r\eta})\right\|^2\right] \der t}_{\text{Term 3}}.
    \end{aligned} 
\end{equation*}
While Novikov's condition may not be met in general, we adopt the approach employed in~\cite{chen2023improved} and sidestep this issue by utilizing a differential inequality argument as shown in Lemma~\ref{lem:prop8_chen2023improved}.
\paragraph{Upper bound Term 2.}
Term 2 corresponds to the discretization error, which has been successfully addressed in previous work~\cite{chen2022sampling,chen2023improved}. By utilizing the unique structure of the Ornstein-Uhlenbeck process, they managed to limit both the time and space discretization errors, which decrease as $\eta$ becomes smaller. To ensure the completeness of our proof, we have included it in Lemma~\ref{lem:dis_err}, utilizing the segmented notation presented in Section~\ref{sec:pre}.
\paragraph{Upper bound Term 3.}
Term 3 represents the accuracy of the score estimation.
In DMs, due to the parameterization of the target density, this term is trained by a neural network and assumed to be less than $\epsilon$ to ensure the convergence of the reverse process.
However, in \ourmethod, the score estimation is obtained using a non-parametric and stochastic approach, i.e., Alg~\ref{con_alg:rse}.
Therefore, we provide a high probability bound for this term under Alg~\ref{con_alg:rse}, which is demonstrated in Lemma~\ref{lem:rse_err}.

Roughly speaking, for each $(k,r)$ pair in Alg~\ref{alg:rrds}, we consider the following probability.
\begin{equation}
    \label{ineq:rse_core}
    \small
    \begin{aligned}
        &\sP\left[\left\|\grad\ln p_{k,S-r\eta}(\vx)- \rbkwv_{k,r\eta}(\vx)\right\|^2\le \epsilon,\forall \vx\in\R^d\right]\\
        & \ge \sP\left[\left\|\grad\ln p_{k,S-r\eta}(\vx)-\rbkwv_{k,r\eta}(\vx)\right\|^2\le \epsilon, \forall \vx\in\R^d \Big| \bigcap_{
            (i,j)\in \sS_{k,r}
        } \left\|\grad\ln p_{k,0}(\vx^\prime_{i,j}) -\rbkwv_{k-1,0}(\vx^\prime_{i,j})\right\|^2\le l_{k,r}(\epsilon)\right]\\
        &\cdot \mathbb{P}\left[\bigcap_{
            (i,j)\in \sS_{k,r}
        } \left\|\grad\ln p_{k,0}(\vx^\prime_{i,j}) -\rbkwv_{k-1,0}(\vx^\prime_{i,j})\right\|^2\le l_{k,r}(\epsilon)\right]\quad \mathrm{where}\quad \sS_{k,r} \coloneqq  \mathbb{N}_{1,n_{k,r}(\epsilon)}\times \mathbb{N}_{0,m_{k,r}(\epsilon)-1}
    \end{aligned}
\end{equation}
When the recursive score estimation, i.e., $\rbkwv_{k-1,0}(\vx^\prime_{i,j})$, is given for each $(i,j)$ pair, Lemma~\ref{lem:recursive_core_lem} provides the upper bound of score estimation error as:
\begin{equation*}
    \small
    \begin{aligned}
        \left\|\rbkwv_{k,r\eta}(\vx) - \grad\ln p_{k,S-r\eta}(\vx)\right\|^2\le  \frac{2e^{-2(S-r\eta)}}{\left(1-e^{-2(S-r\eta)}\right)^2}\cdot \underbrace{\left\|-\frac{1}{n_{r,k}(\epsilon)}\sum_{i=1}^{n_{r,k}(\epsilon)} \rvx_i^\prime + \E_{\rvx^\prime \sim q^\prime_{k,S-r\eta}(\cdot|\vx)}\left[\rvx^\prime\right]\right\|^2}_{\text{Term 3.1}}\\
        \quad + \frac{2e^{-2(S-r\eta)}}{\left(1-e^{-2(S-r\eta)}\right)^2}\cdot \underbrace{\left\|-\E_{\rvx^\prime \sim q^\prime_{k,S-r\eta}(\cdot|\vx)}\left[\rvx^\prime\right] + \E_{\rvx^\prime \sim q_{k,S-r\eta}(\cdot|\vx)}\left[\rvx^\prime\right]\right\|^2}_{\text{Term 3.2}}
    \end{aligned}
\end{equation*}
where $q^\prime_{k,S-r\eta}(\cdot|\vx)$ is the underlying distribution of output particles, i.e., $\rvx^\prime_{m_{k,r}(l(\epsilon))}$ in Alg~\ref{con_alg:rse}.
Upper-bounding RHS corresponds to the intuition presented in Fig~\ref{con_fig:rse} and specific steps outlined in Alg~\ref{con_alg:rse}. 
In particular,
\begin{itemize}
    \item Term 3.1 has a high probability $\epsilon$-level upper bound that can be achieved by selecting sufficiently large $n_{k,r}(\epsilon)$, as the concentration probability of $q^\prime_{k,S-r\eta}(\cdot|\vx)$ is demonstrated in Lemma~\ref{lem:thm8_vempala2019rapid}. 
    This corresponds to Step 1 in Fig~\ref{con_fig:rse} and Line 4 in Alg~\ref{con_alg:rse}.
    \item Term 3.2 can be upper bounded by $\KL{q^\prime_{k,S-r\eta}(\cdot|\vx)}{q_{k,S-r\eta}(\cdot|\vx)}$ can be contracted by utilizing the ULA with a sufficiently large iteration count, i.e., $m_{k,r}(\epsilon)$, when the score $\grad\ln p_{k,0}$ is well-approximated. 
    This corresponds to Step 2 in Fig~\ref{con_fig:rse} and Line 6-Line 9 in Alg~\ref{con_alg:rse}.
    \item To upper bound Term 3.2, the accuracy of estimating the score $\grad\ln p_{k,0}$ requires to be less than $l_{k,r}(\epsilon)$ which is implemented by recursion, i.e., Line 7 in Alg~\ref{con_alg:rse}, and corresponds to Step 3 in Fig~\ref{con_fig:rse}.
\end{itemize}
Therefore, Eq~\ref{ineq:rse_core} can be rewritten as:
\begin{equation*}
    \small
    \begin{aligned}
        &\sP\left[\left\|\grad\ln p_{k,S-r\eta}(\vx)- \rbkwv_{k,r\eta}(\vx)\right\|^2\le \epsilon,\forall \vx\in\R^d\right]\ge (1-\delta)\cdot \mathbb{P}\left[\bigcap_{
            (i,j)\in \sS_{k,r}
        } \left\|\grad\ln p_{k,0}(\vx^\prime_{i,j}) -\rbkwv_{k-1,0}(\vx^\prime_{i,j})\right\|^2\le l_{k,r}(\epsilon)\right]\\
        & \ge (1-\delta)\cdot \left(\mathbb{P}\left[\left\|\grad\ln p_{k,0}(\vx^\prime) -\rbkwv_{k-1,0}(\vx^\prime)\right\|^2\le l_{k,r}(\epsilon),\forall \vx^\prime\in\R^d\right]\right)^{\left|\sS_{k,r}\right|}
    \end{aligned}
\end{equation*}
where the last inequality follows from the independence of $\rbkwv_{k-1,0}$ for each $(i,j)$ pair.
We only need to use this proof process recursively like Alg~\ref{alg:rrds} with proper choice of $\delta$ to get the bound as:
\begin{equation*}
    \small
    \sP\left[\bigcap_{
               (k,r)\in\sS_{k,r}
           }\left\|\grad\ln p_{k,S-r\eta}(\tilde{\vx}_{k,r\eta})-\tilde{\rvv}_{k,r\eta}(\tilde{\vx}_{k,r\eta})\right\|^2\le \epsilon\right]\ge 1-\epsilon,
\end{equation*}
which implies $\text{Term 3} \le \tilde{O}(\epsilon)$ with a probability at least $1-\epsilon$.
Due to the large amount of computation, we defer the details of the recursive proof procedure and the choice of $\delta$ to the Appendix.

%---------------Dec. 31st ---------------
%------------Dec. 31--------------
{
    
    \section{Empirical Results}
    
    \noindent\textbf{Problem settings.} We consider the target distribution defined on $\R^2$ to be a mixture of Gaussian distributions with $6$ modals.
    Meanwhile, we draw $1,000$ particles from the target distribution shown in Fig~\ref{fig:gtsamples} and used MMD (with RBF kernel) as the metric.

    \begin{figure}
    \centering
    \includegraphics[width=4.cm]{0_figs/gtsamples.png}
    \vspace{-.1in}
    \caption{The 1000 particles sampled from the target distribution, which utilized as the criterion by using MMD}
    \label{fig:gtsamples}
    \vspace{-.1in}
    \end{figure}

    We compare the MMDs among three sample algorithms including ULA~\cite{neal1992bayesian,roberts1996exponential}, DMC~\cite{huang2023monte}, and \ourmethod\  when the number of gradient oracles are $\{200, 400, 600, 800, 1600, 3200\}$.
    Besides, we tuned hyper-parameters for all three algorithms and left their optimal choice in our code given in the latest supplementary material.
    Then, we show the final MMDs in Fig~\ref{fig:exp}.

    \begin{figure}
    \centering
    \includegraphics[width=9.cm]{0_figs/output.png}
    \vspace{-.1in}
    \caption{\small MMD results for ULA, DMC, and \ourmethod\ for the different gradient complexity. Experimental results show that ULA attains a slow convergence rate with a high sampling error. Both DMC and RS-DMC  converge rapidly but RS-DMC can achieve smaller sampling errors than DMC, even with lower gradient complexities.  In particular, RS-DCM with 800 gradient complexity can outperform DCM with over 3000 gradient complexity.}
    \label{fig:exp}
    \vspace{-.1in}
    \end{figure}

    Besides, to compare the behaviors of the three methods, we illustrate the particles when the algorithms return for different gradient complexity in Fig~\ref{fig:illustration_exp}.
    We note that
    \begin{itemize}
        \item ULA will quickly fall into some specific modals with an extremely high sampling error, measured in Maximum Mean Discrepancy (MMD), and is significantly worse than DMC and \ourmethod.
        \item DMC will quickly cover the different modals. However, converging to their means will be slower than \ourmethod.
        \item \ourmethod will quickly cover the different modes and converge to their means. Compared to DMC, it requires much fewer gradient complexities to achieve a similar sampling error. For instance, RS-DMC with 800 gradient complexity can outperform DMC with over 3200. 
    \end{itemize}
    \begin{figure}
    \centering
    \begin{tabular}{ccc}
          \includegraphics[width=4cm]{0_figs/ULA_200.pdf}&
          \includegraphics[width=4cm]{0_figs/ULA_400.pdf}&
          \includegraphics[width=4cm]{0_figs/ULA_800.pdf}\\
          \includegraphics[width=4cm]{0_figs/DMC_200.pdf}&
          \includegraphics[width=4cm]{0_figs/DMC_400.pdf}&
          \includegraphics[width=4cm]{0_figs/DMC_800.pdf}\\
          \includegraphics[width=4cm]{0_figs/RS-DMC_200.pdf}&
          \includegraphics[width=4cm]{0_figs/RS-DMC_400.pdf}&
          \includegraphics[width=4cm]{0_figs/RS-DMC_800.pdf}\\
          $\mathrm{grad\ num}=200$&$\mathrm{grad\ num}=400$&$\mathrm{grad\ num}=800$\\
          \includegraphics[width=4cm]{0_figs/ULA_1600.pdf}&
          \includegraphics[width=4cm]{0_figs/ULA_3200.pdf}& \\
          \includegraphics[width=4cm]{0_figs/DMC_1600.pdf}&
          \includegraphics[width=4cm]{0_figs/DMC_3200.pdf}& \\
          \includegraphics[width=4cm]{0_figs/RS-DMC_1600.pdf}&
          \includegraphics[width=4cm]{0_figs/RS-DMC_3200.pdf}& \\
          $\mathrm{grad\ num}=1600$&$\mathrm{grad\ num}=3200$&
    \end{tabular}
    \caption{\small Illustration of the returned particles for ULA, DMC, and \ourmethod. The first row is returned by ULA, the second is DMC and the last is from \ourmethod. Experimental results show that ULA converges fast in the local regions of modes, while it suffers from the problem of covering all modes. DMC can cover most modes with few gradient oracles but converge slowly in local regions. \ourmethod\ takes advantage of both ULA and DMC, which can cover most modes and admit a relatively faster local convergence. 
    }
    \label{fig:illustration_exp}
    \end{figure}

    \paragraph{Explanation about the resemblance of modals' variances.}
    In the previous experiments, all parameters were tuned to achieve a lower MMD. However, in some cases, MMD may not be able to perfectly characterize the sampling performance, while some statistical information, e.g., the resemblance of variances of modals may be obfuscated. In order to mitigate this issue, we further conduct the experiments with a different set of hyperparameters such that the generated samples can be reasonably closer to the ground truth. In particular, we set the gradient complexity as $200$ and generate samples using ULA, DMC, and \ourmethod. The distribution of the output particles is visualized in Fig~\ref{fig:ula_dmc_cmp_var}. The comparisons of MMD and variance estimations of different modals are shown in Table~\ref{tab:resemble_mmd} and Table~\ref{tab:resemble_var}, respectively. Then it can be clearly observed that
    \begin{itemize}
    \item \ourmethod has better coverage than ULA and DMC, which is measured by MMD (see Fig~\ref{fig:ula_dmc_cmp_var}  and Table~\ref{tab:resemble_mmd}).
    \item \ourmethod has better concentration than ULA and DMC, which is measured by the variance of modals (see Table~\ref{tab:resemble_var}, where the variance of \ourmethod\ is closer to that of the ground truth samples for almost all modals).
    \end{itemize}

    This again demonstrates the superior performance of \ourmethod compared to baseline algorithms.
    % Actually, it is caused by the MMD criterion rather than DMC and \ourmethod\ algorithm. 
    % We find the output particles have a similar variance with the target distribution under some sub-optimal parameters, and even in this condition, DMC and \ourmethod\ will have a better MMD compared with ULA. 
    % However, these parameters are discarded since they do not give the best MMD. 
    
    
    \begin{table}[b]
        \centering
        \begin{tabular}{c c c c c}
             & ULA & DMC & \ourmethod \\
             \hline
             MMD loss & 1.386 & 0.129 & 0.112\\
             \hline
        \end{tabular}
        \caption{\small The comparison of MMD in the good resemblance of modals' variances when gradient complexity is chosen as $200$.}
        \label{tab:resemble_mmd}
    \end{table}
    
    \begin{table}[!hbpt]
        \centering
        \begin{tabular}{c c c c c}
             Var & ULA & DMC & \ourmethod & ground truth\\
             \hline
             Modal 0 & 0.0337 & 0.0337 & 0.0332 & 0.0217\\
             Modal 1 & 0.0574 & 0.0311 & 0.0314 & 0.0188\\
             Modal 2 & 0.0459 & 0.0299 & 0.0324 & 0.0196\\
             Modal 3 & 0.0394 & 0.0338 & 0.0287 & 0.0184\\
             Modal 4 & 0.0449 & 0.0330 & 0.0289 & 0.0174\\
             Modal 5 & 0.0409 & 0.0321 & 0.0306 & 0.0220\\ 
             \hline
        \end{tabular}
        \caption{\small The comparison of variance of different modals when gradient complexity is chosen as $200$. The experimental results show both DMC and \ourmethod can achieve better variance estimation. In some remote modals, the gap between ULA and DMC/\ourmethod will be even larger than that between \ourmethod and ground truth.}
        \label{tab:resemble_var}
    \end{table}
    
    \begin{figure}
    \centering
    \begin{tabular}{cccc}
          \includegraphics[width=3cm]{0_figs/GT_var_esb.pdf}&
          \includegraphics[width=3cm]{0_figs/ULA_var_esb.pdf}&
          \includegraphics[width=3cm]{0_figs/DMC_var_esb.pdf}&
          \includegraphics[width=3cm]{0_figs/RS-DMC_var_esb.pdf}\\
          ground truth& ULA output & DMC output &RS-DMC output\\
    \end{tabular}
    \caption{\small Distribution of the samples generated by ULA, DMC, and RS-DMC, where the gradient complexity is set to be $200$. 
    }
    \label{fig:ula_dmc_cmp_var}
    \end{figure}

}
